Do you understand epistemic uncertainty? Think again! Rigorous frequentist epistemic uncertainty estimation in regression

Quantifying model uncertainty is critical for understanding prediction reliability, yet distinguishing between aleatoric and epistemic uncertainty remains challenging. We extend recent work from classification to regression to provide a novel frequentist approach to epistemic and aleatoric uncertainty estimation. We train models to generate conditional predictions by feeding their initial output back as an additional input. This method allows for a rigorous measurement of model uncertainty by observing how prediction responses change when conditioned on the model's previous answer. We provide a complete theoretical framework to analyze epistemic uncertainty in regression in a frequentist way, and explain how it can be exploited in practice to gauge a model's uncertainty, with minimal changes to the original architecture.

==> bib/figmacro.tex <==
\newif\ifrgb
\rgbfalse

\newif\iffig
\figtrue

\newcommand{\figx}[2]
{
 \iffig
  \includegraphics[width=#1,keepaspectratio]{#2} 
 \else
   \parbox{#1}{#2} 
 \fi
}

\newcommand{\figy}[2]
{
 \iffig
  \includegraphics[height=#1,keepaspectratio]{#2}  
   \else
  \parbox{#1}{#2} 
 \fi
}

\newcommand{\figxy}[3]
{
 \iffig
  \includegraphics[width=#1,height=#2]{#3} 
 \else
   \parbox{#1}{#2}
  \fi
}

\newcommand{\figurecaption}[2]
{
\caption[]{\parbox[t]{#1}{#2}}
}

\newcommand{\fcaption}[1]
{
 \figurecaption{0.9\linewidth}{\small #1}
}

\newcommand{\figdir}[1]
{
\def\figurepath{#1}
}

\renewcommand{\topfraction}{1}
\renewcommand{\dbltopfraction}{1}
\renewcommand{\bottomfraction}{1}
\renewcommand{\textfraction}{.0}
\renewcommand{\floatpagefraction}{1}
\renewcommand{\dblfloatpagefraction}{1}


==> bib/report.tex <==
\usepackage{named}

\usepackage{geometry}
\usepackage{times}
\usepackage{graphics}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{amsthm,amssymb}
\usepackage{color}

\geometry{
 a4paper,
 left=21mm,
 right=21mm,
 top=16mm,
 bottom=16mm,
 }
 
%\setlength{\oddsidemargin}{0.0in}
%\setlength{\topmargin}{-0.125in}
%\setlength{\textwidth}{6.25in}
%\setlength{\textheight}{8.75in}
%\parskip 6pt plus 3pt minus 2pt

\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\be}{\begin{enumerate}}
\newcommand{\ee}{\end{enumerate}}
\newcommand{\bd}{\begin{description}}
\newcommand{\ed}{\end{description}}
\newcommand{\im}{\item}
\newcommand{\comment}[1]{}
\newcommand{\missing}[1]{\begin{large} {\bf ADD:} {\em #1} \end{large}}
\newcommand{\note}[1]{\begin{center} \noindent\framebox{\begin{minipage}{8cm}{\bf #1}\end{minipage}}\end{center}\\}
\newcommand{\rmk}[1]{{\color{red}{ \bf #1}}}
\newcommand{\red}[1]{{\color{red}{#1}}}
\newcommand{\url}[1]{#1}

\newif\ifsubmit
\submitfalse

\newif\ifdraft
\draftfalse

\newcommand{\dspace}{\renewcommand{\baselinestretch}{1.5}\large\normalsize}
\newcommand{\sspace}{\renewcommand{\baselinestretch}{1.0}\large\normalsize}
\newcommand{\Section}[1]{\section{#1}}
\newcommand{\SubSection}[1]{\subsection{#1}}
\sspace

\renewcommand{\floatpagefraction}{1.0}


==> fig/synthetic.tex <==
% !TEX root = ../main.tex
% !TEX spellcheck = en-US

\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/dataset_simplified.png}
    \caption{The training dataset. On the top, the distribution $p(X)$ used to sample the input points, which is a simple Gaussian with $\E[X]=0$ and $\var[X]=4$. The variance in $Y$ follows the law $\sigma(x)=1.5\exp(-x^2 / 2)$.}
    \label{fig:dataset}
\end{figure*}

==> figures/calibration_idea.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1, scale=0.9]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da4264122997874369] 
\draw   [dashed] (339.5,45) -- (339.5,206) ;
%Curve Lines [id:da6337761343986679] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=1.5]    (259.5,46) .. controls (328.5,258.5) and (349.5,262) .. (420,46) ;
%Curve Lines [id:da8082472298403462] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=1.5]    (260,68.67) .. controls (328.5,291.67) and (374.5,213.5) .. (407,47) ;
%Shape: Square [id:dp009679049835678688] 
\draw  [line width=1.5]  (259.5,46) -- (420,46) -- (420,206.5) -- (259.5,206.5) -- cycle ;
%Straight Lines [id:da0556747417903225] 
\draw    (261.67,219.67) -- (417,220) ;
\draw [shift={(419,220)}, rotate = 180.12] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
\draw [shift={(259.67,219.67)}, rotate = 0.12] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Shape: Rectangle [id:dp7926661072956127] 
\draw  [draw opacity=0][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (334.83,214) -- (343.83,214) -- (343.83,225.67) -- (334.83,225.67) -- cycle ;

% Text Node
\draw (333.67,215.07) node [anchor=north west][inner sep=0.75pt]    {$x$};
% Text Node
\draw (422,212.9) node [anchor=north west][inner sep=0.75pt]    {$+$};
% Text Node
\draw (243.67,212.73) node [anchor=north west][inner sep=0.75pt]    {$-$};
% Text Node
\draw (231.73,144) node [anchor=north west][inner sep=0.75pt]  [rotate=-270]  {$p(y|x)$};
% Text Node
\draw (277,57) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\fontfamily{cmss}\selectfont \textcolor[rgb]{0.29,0.56,0.89}{model}}};
% Text Node
\draw (372.33,56) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\fontfamily{cmss}\selectfont \textcolor[rgb]{0.82,0.01,0.11}{real}}};


\end{tikzpicture}

==> figures/triangle_uncertainties.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Ellipse [id:dp8799922026970501] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.25 ] (390.39,183.14) .. controls (386.29,179.1) and (390.28,168.38) .. (399.32,159.19) .. controls (408.35,150) and (419.01,145.83) .. (423.11,149.86) .. controls (427.21,153.9) and (423.22,164.62) .. (414.18,173.81) .. controls (405.15,183) and (394.49,187.17) .. (390.39,183.14) -- cycle ;
%Shape: Ellipse [id:dp38369231287923466] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.25 ] (385.71,187.9) .. controls (380.43,182.71) and (385.57,168.92) .. (397.19,157.1) .. controls (408.81,145.28) and (422.51,139.91) .. (427.79,145.1) .. controls (433.07,150.29) and (427.93,164.08) .. (416.31,175.9) .. controls (404.69,187.72) and (390.99,193.09) .. (385.71,187.9) -- cycle ;
%Shape: Triangle [id:dp32134381178287064] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.2 ][line width=1.5]  (145.75,97) -- (200.5,190.08) -- (91,190.08) -- cycle ;
%Shape: Triangle [id:dp3396464618476045] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.2 ][line width=1.5]  (284.75,97) -- (339.5,190.08) -- (230,190.08) -- cycle ;
%Shape: Triangle [id:dp8209801933108052] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.2 ][line width=1.5]  (424.25,97.5) -- (479,190.58) -- (369.5,190.58) -- cycle ;
%Shape: Circle [id:dp5929932088108747] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (142.75,97) .. controls (142.75,95.34) and (144.09,94) .. (145.75,94) .. controls (147.41,94) and (148.75,95.34) .. (148.75,97) .. controls (148.75,98.66) and (147.41,100) .. (145.75,100) .. controls (144.09,100) and (142.75,98.66) .. (142.75,97) -- cycle ;
%Shape: Circle [id:dp9914901895398436] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (88,190.08) .. controls (88,188.42) and (89.34,187.08) .. (91,187.08) .. controls (92.66,187.08) and (94,188.42) .. (94,190.08) .. controls (94,191.73) and (92.66,193.08) .. (91,193.08) .. controls (89.34,193.08) and (88,191.73) .. (88,190.08) -- cycle ;
%Shape: Circle [id:dp8369713365158895] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (197.5,190.08) .. controls (197.5,188.42) and (198.84,187.08) .. (200.5,187.08) .. controls (202.16,187.08) and (203.5,188.42) .. (203.5,190.08) .. controls (203.5,191.73) and (202.16,193.08) .. (200.5,193.08) .. controls (198.84,193.08) and (197.5,191.73) .. (197.5,190.08) -- cycle ;
%Shape: Circle [id:dp13689975403825683] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (261.75,167.5) .. controls (261.75,165.84) and (263.09,164.5) .. (264.75,164.5) .. controls (266.41,164.5) and (267.75,165.84) .. (267.75,167.5) .. controls (267.75,169.16) and (266.41,170.5) .. (264.75,170.5) .. controls (263.09,170.5) and (261.75,169.16) .. (261.75,167.5) -- cycle ;
%Shape: Circle [id:dp7009544335636904] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (403.75,166.5) .. controls (403.75,164.84) and (405.09,163.5) .. (406.75,163.5) .. controls (408.41,163.5) and (409.75,164.84) .. (409.75,166.5) .. controls (409.75,168.16) and (408.41,169.5) .. (406.75,169.5) .. controls (405.09,169.5) and (403.75,168.16) .. (403.75,166.5) -- cycle ;
%Shape: Ellipse [id:dp9600803031252321] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.25 ] (395.42,178.03) .. controls (392.57,175.23) and (395.34,167.8) .. (401.6,161.44) .. controls (407.86,155.07) and (415.24,152.18) .. (418.08,154.97) .. controls (420.93,157.77) and (418.16,165.2) .. (411.9,171.56) .. controls (405.64,177.93) and (398.26,180.82) .. (395.42,178.03) -- cycle ;

% Text Node
\draw (81.5,195) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$y_{1}$};
% Text Node
\draw (197,195) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$y_{2}$};
% Text Node
\draw (139,80) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$y_{3}$};
% Text Node
\draw (269.5,150.4) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$p( y)$};
% Text Node
\draw (420.5,169.4) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$p( p( y))$};
% Text Node
\draw (137.5,214.9) node [anchor=north west][inner sep=0.75pt]    {$\mathcal{Y}$};
% Text Node
\draw (273,213.9) node [anchor=north west][inner sep=0.75pt]    {$\Delta _{\mathcal{Y}}$};
% Text Node
\draw (414.5,213.9) node [anchor=north west][inner sep=0.75pt]    {$\Delta _{\Delta _{\mathcal{Y}}}$};
% Text Node
\draw (114,232.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\fontfamily{cmss}\selectfont prediction}};
% Text Node
\draw (247.5,236) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{50.2pt}\setlength\topsep{0pt}
\begin{center}
{\fontfamily{cmss}\selectfont aleatoric}\\{\fontfamily{cmss}\selectfont uncertainty}
\end{center}

\end{minipage}};
% Text Node
\draw (392,236) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{50.2pt}\setlength\topsep{0pt}
\begin{center}
{\fontfamily{cmss}\selectfont epistemic}\\{\fontfamily{cmss}\selectfont uncertainty}
\end{center}

\end{minipage}};


\end{tikzpicture}

==> main_copy.tex <==
% \documentclass{article}
% \usepackage[utf8]{inputenc}
% \usepackage[T1]{fontenc}
% \usepackage{graphicx} % Required for inserting images
% \usepackage{geometry}
% \usepackage{amsfonts,amsmath,amssymb, amsthm}
% \usepackage{dsfont} % funny 1 for indicator func
% \usepackage[dvipsnames]{xcolor}
% \usepackage{tikz}
% \usepackage{textgreek}
% \usepackage{appendix}
% \usepackage[most]{tcolorbox}
% \usepackage{lmodern} 
% \usepackage{hyperref}
% \usepackage{theoremref}
% \usepackage{wrapfig}
% \usepackage{tikz-cd}
% % \usepackage{MnSymbol} % for llangle and rrangle symbols
% \usepackage{mathrsfs} % more cool calligraphic font
% \usepackage{bbold}
% \usepackage{csquotes}
% %\usepackage[
% %backend=biber,
% %style=alphabetic,
% %sorting=ynt,
% %doi=false,
% %url=false
% %]{biblatex}
% %\addbibresource{references.bib}

% % ===== Colors =====
% \definecolor{thmRed}{rgb}{0.502, 0.0, 0.1255}

% % ===== Theorem environments =====
% \newtcolorbox{mydefinition}[2][%
%     enhanced, 
%     breakable,
%     ]{colback=yellow!10!white, colframe=yellow!50!black, fonttitle=\bfseries, title=Definition #2 #1}

% \newtcolorbox{mytheorem}[2][%
%     enhanced, 
%     breakable,
%     ]{colback=thmRed!10!white, colframe=thmRed, fonttitle=\bfseries, title=Theorem #2 #1}

% % Setup counters for theorems and definitions, by section
% \newcounter{theoremCounter}[section]
% \newcounter{definitionCounter}[section]

% % Customize the numbering scheme for theorems and definitions
% \renewcommand{\thetheoremCounter}{\thesection.\arabic{theoremCounter}}
% \renewcommand{\thedefinitionCounter}{\thesection.\arabic{definitionCounter}}

% % Theorem environment
% \newenvironment{theorem}[1][]{%
%     \refstepcounter{theoremCounter}%
%     \mytheorem[#1]{\thetheoremCounter}%
% }{\endmytheorem}

% % Definition environment
% \newenvironment{definition}[1][]{%
%     \refstepcounter{definitionCounter}%
%     \mydefinition[#1]{\thedefinitionCounter}%
% }{\endmydefinition}

% % For section numbering
% \setcounter{secnumdepth}{3}

% % ===== More environments =====
% \newtcolorbox{secabstract}[1][]{colback=RoyalBlue!10!white,
%                                   colframe=RoyalBlue!50!black,
%                                   fonttitle=\bfseries,
%                                   title=Abstract,
%                                   fontupper=\small, #1}
% \newtcolorbox{digressione}[1][%
%     enhanced, 
%     breakable,
%     ]{
%     colback=Gray!10!white,
%     colframe=Gray!50!black,
%     fonttitle=\bfseries,
%     title=Digression,
%     fontupper=\small, #1
%     }


% \renewcommand{\mathsf}[1]{\textsf{#1}} % resolve conflict with mathrsfs package

% % ===== Set up hyperlinks =====
% \hypersetup{
%     colorlinks=true,
%     linkcolor=RoyalBlue,
%     filecolor=RoyalBlue,      
%     urlcolor=RoyalBlue,
%     citecolor=RoyalBlue,
%     pdftitle={Bibliographic Report},
%     pdfpagemode=FullScreen,
%     }

% % ===== Useful commands ===== 
% \input{defs}
% \newcommand{\ent}{\mathbb{H}}
% \newcommand{\E}{\mathbb{E}}
% \newcommand{\C}{\mathbb{C}}
% % \newcommand{\var}{\mathbb{V}\text{ar}}
% \newcommand{\var}{\mathbb{V}}
% \newcommand{\x}{\mathbf{x}}
% \newcommand{\weight}{\boldsymbol{\theta}}
% % \newcommand{\bs}{\boldsymbol}
% \newcommand{\bs}{\mathbf}
% \renewcommand{\deg}{\mathsf{deg}}
% \newcommand{\inspace}{\mathbb R^{c_\text{in}}}
% \newcommand{\outspace}{\mathbb R^{c_\text{out}}}
% \newcommand{\R}{\mathbb{R}}
% \renewcommand{\d}{\mathrm{d}}

% \title{\textsc{Cheat variance: math math math}}
% \author{Enrico Foglia}
% \date{September 2024}

% \begin{document}

% \maketitle

% \begin{abstract}
% \input{sections/00_abstract}
% \end{abstract}

% \section{Introduction}
% \input{sections/01_intro}

% \section{Related work}\label{sec:sota}
% \input{sections/06_related_work}

% \section{Epistemic and Aleatoric Regression Uncertainty}
% \label{sec:math}
% \input{sections/02_math}

% \section{A simple experiment}\label{sec:experiment}
% \input{sections/03_experiments}

% \section{Conclusions}
% \input{sections/04_conclusions}

% \clearpage

% %\bibliographystyle{ICML_2025/icml2025}
% \bibliographystyle{plain}
% \bibliography{bib/string,bib/vision,bib/stats,bib/references}

% \end{document}

==> sections/f-variances.tex <==
\section{Extension to $f$-variances}
It might be useful, at times, to generalize the notion of variance beyond the usual mean square error definition. This leads to the definition of $f$-variance as:
\begin{definition}\label{def:f-variance}
    Let $X,Y:\Omega\to\R$ be random variables and $f:\R\to\R$ a function. The $f$-variance of $X$ is defined to be:
    \begin{equation}
        \var^f[X] = \E[f(X)] - f(\E[X])
    \end{equation}
    Furthermore, let $f':\R^2\to\R$, such that $f'(t,t)=f(t)$. The $f$-covariance is defines as:
    \begin{equation}
        \C^f[X,Y] = \E[f'(X,Y)] - f'(\E[X],\E[Y])
    \end{equation}
\end{definition}
%
if $f$ is convex the $f$-variance is positive by Jensen's inequality. Setting $f(t)=t^2$ and $f'(s,t)=s\cdot t$ recovers the classical definition of variance and covariance. The stringency of the hypothesis of distribution calibration allows to extend most of the results of the present paper to general $f$-variances, starting from Thm.~\ref{tmh: model moments}:
\begin{theorem}
    Let $p_\theta(Y\vert X)$ be distribution calibrated. Then:
    \begin{equation}
    \begin{aligned}
          \mu_\theta(x) &\triangleq \E_\theta[Y\vert x] = \E[\E[Y\vert X]\vert [x]]\\
        \sigma_\theta^f(x) &\triangleq \var^f_\theta[Y\vert x] = \E[\var^f[Y\vert X]\vert [x]] + \var^f[\E[Y\vert X]\vert [x]]
    \end{aligned}
    \end{equation}
\end{theorem}
\begin{proof}
    \begin{equation}
        \begin{aligned}
            \var^f_\theta[Y\vert x] &= \E_\theta[f(Y)\vert x]-f(\E_\theta[Y\vert x])\\
            &=\E[\E[f(Y)\vert X]\vert [x]] - f(\E[\E[Y\vert X]\vert [x]])\\
            &=\E[\E[f(Y)\vert X]\vert [x]]-\E[f(\E[Y\vert X])\vert [x]] - f(\E[\E[Y\vert X]\vert [x]])+\E[f(\E[Y\vert X])\vert [x]]\\
            &=\E[\var^f[Y\vert X]\vert [x]] + \var^f[\E[Y\vert X]\vert [x]]
        \end{aligned}
    \end{equation}
\end{proof}
Thus the same decomposition into aleatoric and epistemic uncertainty apply even to more general forms of variance. The epistemic variance $\var^f[\E[Y\vert X]\vert[x]]$ can be recovered by using a model $p_\theta(y_1,y_2\vert x)$ calibrated on pairs by computing the $f$-covariance between the two responses of the model:
\begin{theorem}
    Let $p_\theta(Y_1,Y_2\vert X)$ be distribution calibrated at predicting pairs. Then:
    \begin{equation}
        \cov_\theta^f(x)\triangleq \C_\theta^f[Y_1,Y_2\vert x] \geq \var^f[\E[Y\vert X]\vert[x]]
    \end{equation}
\end{theorem}

\begin{proof}
    \begin{equation}
        \begin{aligned}
            \C_\theta^f[Y_1,Y_2\vert x] &= \E_\theta[f'(Y_1,Y_2)\vert x] - f'(\E_\theta[Y_1\vert x],\E_\theta[Y_2\vert x])&\text{def.~\ref{def:f-variance}}\\
            &=\E[\E[f'(Y_1,Y_2)\vert X]\vert[x]]-f'(\E[\E[Y_1\vert X]\vert[x]], \E[\E[Y_2\vert X]\vert[x]])&\text{def.~\ref{def:calibration}}\\
            &=\E[\E[f(Y)\vert X]\vert[x]]-f(\E[\E[Y\vert X]\vert[x]])&\text{$Y_1\vert X$ and $Y_2\vert X$ are iid}\\
            &\geq \E[f(\E[Y\vert X])\vert [x]] - f(\E[\E[Y\vert X]\vert[x]])&\text{Jensen's inequality}\\
            &=\var^f[\E[Y\vert X]\vert [x]]&\text{def.~\ref{def:f-variance}}
        \end{aligned}
    \end{equation}
\end{proof}

